Effects of Rotation on the Spectra of Brown Dwarfs

Measured rotational speeds of giant planets and brown dwarfs frequently constitute appreciable fractions of the breakup limit, resulting in centrifugal expansion of these objects at the equator. According to models of internal energy transport, this expansion ought to make the poles of a rotator significantly hotter than the equator, so that inclination of the rotational axis greatly affects both spectral shape and total flux. In this article, we explore the dependence of a substellar object's observables on its rotational speed and axis inclination. To do so, we combine PICASO (a Planetary Intensity Code for Atmospheric Spectroscopy Observations) with software PARS (Paint the Atmospheres of Rotating Stars). The former computer program models radiative transfer within plane-parallel planetary atmospheres, while the latter computes disk-integrated spectra of centrifugally deformed gaseous masses. We find that the specific flux of a typical fast-rotating brown dwarf can increase by as much as a factor of 1.5 with movement from an equator-on to a pole-on view. On the other hand, the distinctive effect of rotation on spectral shape increases toward the equator-on view. The latter effect also increases with lower effective temperature. The bolometric luminosity estimate for a typical fast rotator at extreme inclinations has to be adjusted by as much as about 20% due to the anisotropy of the object's observed flux. We provide a general formula for the calculation of the corresponding adjustment factor in terms of rotational speed and inclination.

==> table_aas.tex <==
\begin{deluxetable*}{lccccr}
\tablecaption{Parameters of our three main substellar models. }
\tablehead{
    Name & 
    J0348-6022 (Model 880) & 
    J0407+1546 & 
    $\beta$ Pictoris b}
\startdata
Parameters Reference & \cite{Tannock_2021AJ} & \cite{Tannock_2021AJ} & \cite{Chilcote_2017AJ} \\
Spectral Type & T7 & L3.5 & L2 \\
$\mathbf{M\,(M_{\rm Jup})}$ & \textbf{42.9} & \textbf{67.0} & \textbf{12.9} \\
$\mathbf{R_{\rm e}\,(R_{\rm Jup})}$ & \textbf{0.905} & \textbf{0.973} & \textbf{1.46} \\
$\bar{T}_{\rm eff}\,({\rm K})$ & 880 & 1840 & 1724 \\ 
$P_{\rm rot}\,({\rm h})$ & 1.08 & 1.23 & \\
$v \equiv v_{\rm e}\sin{i}\,{\rm (km/s)}$ & & & 25\\
$i$ & & &${\pi/2}$\tablenotemark{a}\\
$f \equiv \frac{R_{\rm e} - R_{\rm p}}{R_{\rm e}}$ & 0.08 & 0.05 & 0.029\tablenotemark{b} \\
\hline
$R_{\rm avg} \equiv \frac{R_{\rm e} + R_{\rm p}}{2} ~(R_{\rm Jup})$ & 0.869 & 0.949 & 1.44\\
${\bf L} = 4 \pi R_{\rm avg}^2 \sigma_{\rm SB} \bar{T}_{\rm eff}^4 ~ {\bf (L_\odot)}$ & ${\bf 4.3\times10^{-6}}$ & ${\bf 9.8\times10^{-5}}$ & ${\bf 1.7\times10^{-4}}$\\
$\Omega = 2\pi/P_{\rm rot}~({\rm rad\,s^{-1}})$ & $0.0016$ & $0.0014$ & \\
$\Omega = v / (R_{\rm e}\,\sin{i})~({\rm rad\,s^{-1}})$ & & & $0.00024$\\
$\Omega_{\rm K} = \sqrt{GM/R_{\rm e}^3}~({\rm rad\,s^{-1}})$ & $0.0045$ & $0.0050$ & $0.0012$\\
$\omega = \Omega / \Omega_{\rm K}$ & $0.36$ & $0.28$ & $0.20$\\
$\mathbb{C} = C/(MR_{\rm e}^2) $ & $0.20$\tablenotemark{c} & & $0.25$\tablenotemark{d}\\
${\bf \boldsymbol\omega_{\rm R} = 2\,f / (1 - f)}$\tablenotemark{e} & ${\bf 0.42}$ & ${\bf 0.32}$ & ${\bf 0.24}$
\enddata
\tablenotetext{a}{Assuming that the direction of the brown dwarf's spin angular momentum is the same as those of its star's spin, orbital, and circumstellar disk angular momenta \citep[e.g.,][]{Kraus_2020ApJ}.}
\tablenotetext{b}{From $\omega$ and the Darwin-Radau relation, assuming $\mathbb{C}=0.25$.}
\tablenotetext{c}{Computed from $f$ and $\omega$ according to Equation \eqref{eq:C}.}
\tablenotetext{d}{Similar to estimates for Jupiter \citep{Ni_2018AA} and Saturn \citep{Fortney_2018book}.}
\tablenotetext{e}{Dimensionless rotational velocity $\omega$ corresponding to oblateness $f$ under the Roche model.}
\label{tab:bd_params}
\end{deluxetable*}

